Copyright Protection in Generative AI: A Technical Perspective

Generative AI has witnessed rapid advancement in recent years, expanding their capabilities to create synthesized content such as text, images, audio, and code. The high fidelity and authenticity of contents generated by these Deep Generative Models (DGMs) have sparked significant copyright concerns. There have been various legal debates on how to effectively safeguard copyrights in DGMs. This work delves into this issue by providing a comprehensive overview of copyright protection from a technical perspective. We examine from two distinct viewpoints: the copyrights pertaining to the source data held by the data owners and those of the generative models maintained by the model builders. For data copyright, we delve into methods data owners can protect their content and DGMs can be utilized without infringing upon these rights. For model copyright, our discussion extends to strategies for preventing model theft and identifying outputs generated by specific models. Finally, we highlight the limitations of existing techniques and identify areas that remain unexplored. Furthermore, we discuss prospective directions for the future of copyright protection, underscoring its importance for the sustainable and ethical development of Generative AI.

==> sections/problem_statement.tex <==

\section{Background}

Deep Generative Models (DGMs) is a branch of deep learning, focusing on data generation. DGMs try to learn real data distribution $p_{\text{data}}$ usually by optimizing the parameters $\theta$ of the deep neural networks. After learning an approximate distribution, a new data is commonly generated by sampling from a random distribution or a conditional distribution. Due to the widespread application of models such as GAN, Diffusion Model, and transformer in recent years, the studies on copyright protection mainly focused on these models. So in this part, we will introduce Deep Generative Models for image generation and text generation respectively, especially the models with much research on copyright protection.

%\jr{I think in this paragraph, we first demonstrate what does DGM do (generate by learning a distribution), what is the real distribution and DGM tries to use a learned distribution to approximate it. Then what is the category and the comment on the category above.}


% \jt{BTW, leave anything you want others to see in PDF, instead of comments.}



\subsection{Image generation}

\jr{Give a paragraph to introduce what do you do in section 2.1.
}
\jz{I think "Category and examples in image" is a little strange, so I use "DGMs for image generation"}
\subsubsection{Generative Adversarial Network}
Generative Adversarial Network (GAN)\citep{goodfellow2014generative} is proposed in 2014, and first achieved success in synthesizing convincing images. 

In GAN, there are two components, discriminator $D$ and generator $G$, and both of them are usually built with deep neural networks. \jr{I think there are no paper say adversarial training, you can look at the other surveys, how do you get this word? Because adversarial training is confused with adversarial attack and defense}. The generator $G$ captures the real data distribution $p_{\text{data}}$, and can map an arbitrary noise distribution $p_ {\boldsymbol{z}}$ to the real data distribution. The goal of discriminator $D$ is accurately determining whether a sample is from real data distribution or generated by the generator $G$. \jr{(This concept is not mentioned before your use it, just like it is not defined before you use it in your code. You can say GAN has two components, discriminator D and generator G, discriminator do what what, G do what what).} While the discriminator $D$ is trained to distinguish the real data from the data generated by $G$, the generator $G$ is trained simultaneously to generate data that fools $D$.\jz{I rewrite this sentence, firstly to introduce the loss function.} \jr{(Why are they opposite, I think it is not clear.)} \jr{(make the name correct and consistent)} \jr{(D cannot determine the source of a sample doesn't only mean G can generate similar samples, it is also possible that D is just bad. Here just say converge to G can generate good sample that D cannot distinguish. And I think we should mention the loss function before this converge)} By optimizing the loss function below through multiple rounds, the generator $G$ will be improved to generate data that follows the distribution of the real data. \jz{I don't know whether what I write is enough. I avoid the problem that "D cannot determine the source of a sample doesn't only mean G can generate similar samples, it is also possible that D is just bad." I just say it can be improved. And that problem is a challenge to train the GAN, need we say challenge? If we need, I will add.} 

\begin{equation}\label{eq: gan}
    \begin{aligned}
    \min _G \max _D \mathbb{E}_{\boldsymbol{x} \sim p_{\text{data}}(\boldsymbol{x}) } \log D(\boldsymbol{x}) +\mathbb{E}_{\boldsymbol{z} \sim p_{\boldsymbol{z}}(\boldsymbol{z})} \log (1-D(G(\boldsymbol{z})))
    \end{aligned}
\end{equation}
where $D(\cdot)$ is the output of the discriminator, the range of values is within $[0, 1]$, and $G(\cdot)$ is the output of the generator, $\boldsymbol{x}$ is the data follows the real data distribution, $\boldsymbol{z}$ is the noise follows $p_ {\boldsymbol{z}}$.


\subsubsection{VAE}
Variational Auto Encoder(VAE) \citep{kingma2013auto} is proposed in 2013 and has a similar structure to Auto Encoder. Auto Encoder is an unsupervised algorithm to learn a latent space to embed the original data. Auto Encoder has two components, encoder and decoder, usually built with neural networks. The encoder maps the origin data $\boldsymbol{x}$ to $\boldsymbol{z}$, $\boldsymbol{z}$ is in a latent space and usually has a lower dimension than $\boldsymbol{x}$. The decoder maps $\boldsymbol{z}$ back to the origin space. The reconstructed data $\boldsymbol{x}\prime$ should be as consistent as possible with $\boldsymbol{x}$. Although it is possible to generate a new data by generating a random $\boldsymbol{z}$ and placing it in the decoder, it is difficult to generate vectors that follow the late space, so the result is not good. Instead of learning a latent space, VAE learns a new distribution for each feature. Each feature is described using a Gaussian distribution so the output of the encoder is $d_{\boldsymbol{z}}$ means and $d_{\boldsymbol{z}}$ variances where $d_{\boldsymbol{z}}$ is the dimension of $\boldsymbol{z}$. And the latent code $\boldsymbol{z}$ is sampled from the distribution randomly. And then new data can be generated by the decoder. The loss function is
\begin{equation*}\label{eq: vae}
    \begin{aligned}
    \mathcal{L} _{VAE}=-\mathbb{E} _{\boldsymbol{z}\sim Q\left( \boldsymbol{z}|\boldsymbol{x} \right)}\log P\left( \boldsymbol{x}|\boldsymbol{z} \right) +KL\left( Q\left( \boldsymbol{z}|\boldsymbol{x} \right) \parallel P\left( \boldsymbol{x} \right) \right) 
    \end{aligned}
\end{equation*}
where $Q(\boldsymbol{z}|\boldsymbol{x})$ is the encoder and $P(\boldsymbol{x}|\boldsymbol{z})$ is the decoder, $P(\boldsymbol{z})$ is the prior distribution of $\boldsymbol{z}$, $KL(\cdot\parallel\cdot)$ is the Kullback-Leibler divergence.
\subsubsection{Diffusion models}
Diffusion Models were first proposed in 2015 \citep{sohl2015deep}, and have become an emerging generative paradigm which have strong capabilities especially in the image domain. The main idea is from non-equilibrium statistical physics. Diffusion models consist of two stages, namely, a forward process and a reverse process, both of which are modeled as Markov chains. The forward process is to gradually convert a real data $\boldsymbol{x}_0$ which follows the real data distribution to $\boldsymbol{x}_T$ which tends to follow an isotropic normal distribution by $T$ steps. For each step, we can add a noise (i.e., generally Gaussian noise) to the previous data. And then train the reverse process to recover the original input data $\boldsymbol{x}_0$ from the noise by optimizing the usual variational bound on negative log likelihood.
\jr{The structure of this paragraph is fine, but the content is very unclear. Please re-organize the words. You can can read Section 1 and 2.2 in Generative Diffusion Models on Graphs: Methods and Applications, and Applendix C.4 in diffusionshield: A Watermark for Data Copyright Protection against Generative Diffusion Models}

Denoising Diffusion Probabilistic Model (DDPM) \citep{ho2020denoising} made some improvements to diffusion models. Like Diffusion Models, DDPM consists of a forward process $q(\boldsymbol{x}_t|\boldsymbol{x}_{t-1})$ where $\boldsymbol{x}_{t-1}$ is the input of the $t$-th step, and $\boldsymbol{x}$ is the output, and a reverse process $p_{\theta}(\boldsymbol{x}_{t-1}|\boldsymbol{x}_t)$. The forward process is to add a Gaussian noise for each step and the reverse step is a learnable denoising process to recover the origin input data, these process can be described respectively as:
\begin{equation*}\label{eq: ddpm}
    \begin{aligned}
   q(\boldsymbol{x}_t|\boldsymbol{x}_{t-1}) & = \mathcal {N}(\boldsymbol{x}_{t};\sqrt{1-\beta_t}\boldsymbol{x}_{t-1},\beta_t\mathbf{I})\\
    p_{\theta}(\boldsymbol{x}_{t-1}|\boldsymbol{x}_t) & = \mathcal {N} (\boldsymbol{x}_{t-1};\mu_\theta (\boldsymbol{x}_{t},t), {\textstyle \sum_{\theta}}(\boldsymbol{x}_{t},t))
    \end{aligned}
\end{equation*}
where $\beta _t$ is the variance schedule, $\mu_\theta (\boldsymbol{x}_{t},t)$ is the prediction of the mean of $\boldsymbol{x}_{t-1}$ and $\sum_{\theta}$ is the variance. To parameterize $\mu_\theta$ effectively, DDPM predicts the noise $\boldsymbol{\epsilon}_{t}$ added to $\boldsymbol{x}_{t-1}$ instead of directly predicting $\boldsymbol{x}_{t-1}$. And \citet{ho2020denoising} suggest that using the simplified objective as following:
\begin{equation*}\label{eq: ddpm_loss}
    \begin{aligned}
    \mathcal{L}_{DDPM} = \mathbb{E}_{t,\boldsymbol{x}_0,\boldsymbol{\epsilon}_{t}}\left [\left \| \boldsymbol{\epsilon}_{t}-\boldsymbol{\epsilon}_{\theta}\left ( \sqrt{\bar{\alpha}_t\boldsymbol{x}_0}+\sqrt{1-\bar{\alpha}_t}\boldsymbol{\epsilon}_{t},t\right )) \right \| ^{2}\right ] 
    \end{aligned}
\end{equation*}
where $\boldsymbol{\epsilon}_{\theta}$ is the prediction of $\boldsymbol{\epsilon}_{t}$, $\hat{\alpha}_t =  {\textstyle \prod_{s=1}^{t}}(1-\beta_s) $. 

\citet{song2020score} proposed Score-based Generative Model which extends the forward process and reverse process from discrete diffusion steps to continuous scenarios.The forward process and reverse process are modeled by Stochastic Differential Equations (SDE).\jz{Though the outline I write Score-based Diffusion Model, but other survey and the origin paper use Score-based Generative Model, so I use Generative instead of Diffusion. Is that OK?} 
The forward process in infinitesimal time can be described by the following formula:
\begin{equation*}\label{eq: sgm_forward}
    \begin{aligned}
    \mathrm{d}\boldsymbol{x}=\boldsymbol{f} \left( \boldsymbol{x},t \right) \mathrm{d}t+g\left( t \right) \mathrm{d}\boldsymbol{w}
    \end{aligned}
\end{equation*}
where $\boldsymbol{w}$ is the standard Wiener process (a.k.a., Brownian motion), $\boldsymbol{f}(\cdot,\cdot)$ is drift coefficient, a vector-valued function, and $g(\cdot)$ is diffusion coefficient, a scalar function. And the reverse process can be described by the reverse-time SDE:
\begin{equation*}\label{eq: sgm_reverse}
    \begin{aligned}
    \mathrm{d}\boldsymbol{x}=\left[ \boldsymbol{f}\left( \boldsymbol{x},t \right) -g\left( t \right) ^2\nabla _{\boldsymbol{x}}\log p_t\left( \boldsymbol{x} \right) \right] \mathrm{d}t+g\left( t \right) \mathrm{d}\bar{\boldsymbol{w}}
    \end{aligned}
\end{equation*}
where $\bar{\boldsymbol{w}}$ is a standard Wiener process when time flows backwards from $T$ to 0, $\nabla _{\boldsymbol{x}}\log p_t\left( \boldsymbol{x} \right)$ is score of marginal distribution, the only unknown information in reserve-time SDE. To estimate score function, we can train a time-dependent score-based model $\boldsymbol{s}_{\boldsymbol{\theta}(\boldsymbol{x},t)}$ by optimizing:
\begin{equation*}\label{eq: sgm_loss}
    \begin{aligned}
     \mathbb{E}_{t,\boldsymbol{x}_0, \boldsymbol{x}_t} \left [ \lambda (t) \left \| s_\theta(\boldsymbol{x}_t,t) -\nabla _{\boldsymbol{x}_t}\text{log}p_{0t}(\boldsymbol{x}_t |\boldsymbol{x}_0) \right \|^2 \right ]
    \end{aligned}
\end{equation*}
where $\lambda$ is a positive weighting function, $p_{0t}(\boldsymbol{x}_t |\boldsymbol{x}_0)$ is the probability distribution of $\boldsymbol{x}_t$ conditioned on $\boldsymbol{x}_0$, $t$ is uniformly sampled over $[0,T]$, $\boldsymbol{x}_0 \sim p_0(\boldsymbol{x})$, $\boldsymbol{x}_t \sim p_{0t}(\boldsymbol{x}_t | \boldsymbol{x}_0)$.
\jr{For this section 3.1.3, we can just learn and imitate from the two papers I mentioned above.}

Latent diffusion model (LDM) \citep{rombach2022high} first uses a pre-trained Auto-Encoder to convert image pixels to a smaller latent space $\boldsymbol{z}=\varepsilon (\boldsymbol{x})$, and then performs traditional diffusion model inference and optimization. This training method balances the computational power and performance of LDM, speed up the generation of high-resolution image. Specifically, it learns the distribution in latent space, and samples from the latent space then maps it back to the image space. The loss function is
\begin{equation*}
    \begin{aligned}
    \mathcal{L} _{LDM}=\mathbb{E} _{t,\varepsilon \left( \boldsymbol{x} \right) ,\boldsymbol{\epsilon }}\left[ \left\| \boldsymbol{\epsilon }-\boldsymbol{\epsilon }_{\theta}\left( \boldsymbol{z}_t,t \right) \right\| _{2}^{2} \right]
    \end{aligned}
\end{equation*}
\jz{I think Stable Diffusion means this project: https://github.com/CompVis/stable-diffusion.}
Stable Diffusion is based on \citet{rombach2022high}. The input is a text prompt $y$ and the output is an image related to the input text. To achieve this objective, \citet{rombach2022high} augment underlying U-Net backbone with the cross-attention mechanism. It uses a frozen CLIP\citep{Radford2021LearningTV} text encoder to transfer $y$ to the text embedding. And the text embedding is coupled with the U-Net structure in the form of cross-attention, so that each input of image information is fused with text information for training.
\jz{I think to introduce stable-diffusion clearly, I need to introduce Conditioning Mechanisms.} 

\subsection{DGMs for text generation}
With the emergence of transformer architecture\citep{Vaswani2017AttentionIA} in recent years, Language Models (LMs) such as ChatGPT \citep{Ouyang2022TrainingLM} have achieved impressive performance in the field of text generation. Transformer follows an encoder-decoder structure using stacked self-attention and point-wise, fully connected layers. \jz{If we use a picture may be more easy to explain transformer.} The transformer architecture consists of two components: transformer encoder and transformer decoder. The transformer encoder is composed of a stack of several identical layers, each layer consists a multi-head self-attention and a feed-forward layer, also includes layer normalization and residual connection. The transformer decoder is also composed of a stack of several identical layers. Compared to the encoder, each decoder layer includes an additional multi-head
attention layer which accept output from the encoder.
\jz{This part I will introduce GPT. I find that our survey mention GPT-2, ChatGPT-3.5, GPT-4 below. Llama, BERT is not mentioned. So, this part I think I'll introduce GPT series. Copilot is a modified, production version of GPT-3, so will be introduced here.}

\jz{This part may be not very well, I will find some survey if they introduce LLMs briefly, I'll imitate.}
\citep{Radford2018ImprovingLU} explore a self-supervised method to train GPT, using a combination of unsupervised pre-training and supervised fine-tuning. In the pre-training stage, it uses transformer encoder architecture to maximize likelihood function of sentences. In the fine-tuning stage, maximize classification objective function together with likelihood function of sentences to complete classification tasks. The model structure of GPT-2\citep{Radford2019LanguageMA} is basically similar to GPT. But from a new perspective, zero-shot, GPT-2 achieve promising and competitive results in some tasks. In the subsequent work, Open AI uses larger scale of models and more data to improve text generation capabilities, adds code datasets to enhance code generative capabilities and aligns the model by Reinforcement Learning from Human Feedback (RLHF) and Supervised Fine-Tuning (SFT) to reduce the generation of harmful results. GPT-3.5, ChatGPT, GPT-4 has been released. Copilot, a modified version of GPT-3, is a tool to assistant users to code and it has also been widely used.

\jz{Maybe we need not introduce StarBase and StarCoder, just cite at where we use?}


\subsection{DGMs for other domain generation}
Apart from generation in image and text domain, DGMs are also widely used to generate other domain data such as graph and audio data. In graph domain, as a lot of data exists in the form of graphs, such as chemical structures, relational networks, many models are proposed to generate specific types of data. \jz{need we cite some paper to list some examples?} \jr{Yes} And in audio domain, GAN and VAE are used for zero-shot scenario which synthesize a novel unseen voice, and Diffusion Models are used  for few-shot scenario which aims at generating the voice of the target speaker to repeat a specific sentence with only few recordings. Find the model they use in Part 5 and mention them here and also in part 5. \jz{This part do we need to generate a specific paper? In Part 5, we do not mention specific model.}


==> sections/unused.tex <==
\section{Problem Statement \jr{Background. may be better}}

\jt{Process of copoyright protection for intro}

\jr{For this section, I think we can find a survey and imitate their structure to introduce generative model.}
\subsection{Definitions and Notations}
\jr{Do we need this section. At least the title is not consistent with the content. Here in this subsection we can just mention what we will do in Section 2. In the following we can b}
Probabilistic Generative Model, abbreviated as Generative Model, is a model used to generate randomly observable data. Assuming in a high-dimensional space $\mathcal{X}$, data follows a certain distribution $p_r(\boldsymbol{x})$, the Generative Model is based on observable samples $\boldsymbol{x}^{(1)}, \boldsymbol{x}^{(2)}, \dots, \boldsymbol{x}^{(N)}$ to learn a parameterized model $p_\theta(\boldsymbol{x})$. \jr{I think here we should make it clear that $p$ is distribution instead of model, $\theta$ is model parameter.} The small number $n$ in the parentheses in the upper right corner of the variable represents the $n$-th of the $N$ samples. \jr{You can say $\boldsymbol{x}^{(1)}, \boldsymbol{x}^{(2)}, \dots,\boldsymbol{x}^{(2)}, \dot, \boldsymbol{x}^{(N)}$, where $i$ is xxx. Also, I think we don't need to mention the order of samples. Here we don't need to introduce $i$. We should introduce what is $N$. And don't use \textbf{small number} you can use lower-case. Also, we don't need to say it out. Because people can tell the difference between $n$ and $N$} $\boldsymbol{x}$ represents data in a certain domain. Training process is to use samples to let $p_\theta(\boldsymbol{x})$ approach $p_r(\boldsymbol{x})$ which means the generated data is similar to the real data.  Deep generative model is to utilize the ability to approximate arbitrary functions of deep neural network to model a complex distribution $p_r(\boldsymbol{x})$ or directly generate the samples which conform to distribution $p_r(\boldsymbol{x})$.

\jt{outline: In the Section 2, we can use 2.1. 
 for the overall concept of generative model which is like you mentioned to learn a distriobution above. 2.2 category and examples in image. 2.3 category in text, especially LLM. 2.4 other domains but do not make it too detailed}



\subsection{Deep Generative Models}
Deep Generative Models have been in the front edge of deep learning especially since the breakthrough of Diffusion-based Model and Large-Language Model. DGMs learn the probabilistic distribution of dataset and sample from the distribution to generate data. \jr{Because of the ability to learn the distribution, people also make use of DGMs for some discriminative tasks in the beginning. (I think we don't need to mention it)} But with the increasingly advance in generating data, more attention is paid on the generative tasks. In this subsection, we first introduce the \textbf{general designs and frameworks} of different kinds of generative models, then introduce the common generative models in the image, text, video, audio and graph domains briefly for each kind of models.

\jr{The following is too short to make it a paragraph.}
Deep generative models can be divided into 4 categories from different frameworks perspective, Auto-regressive Models, Flow-based Models, Latent Variable Models and Energy-Based Models.


\subsubsection{Auto-regressive Models.} 

Auto-regression is a time series model that uses observations from previous time steps as input to a regression equation to predict the value at the next time step. When used to generate tasks, this kind of model first generates an initial value, and then uses all the previously generated content each time to predict the next moment's content. For $d$-dimensional data $\boldsymbol{x}$, when the model generates $t$-th dimensional data $x_i$, use $\boldsymbol{x}_{1:i-1}$ \jr{When any new notation is given, you have to introduce what it is} as the input of the model to predict. From a modeling perspective, it models data $\boldsymbol{x}$ by $p(\boldsymbol{x})=p(x_1){\textstyle \prod_{i=2}^{d} p(x_i|\boldsymbol{x}_{1:i-1})}$.

In \textbf{image domain}, \citet{van2016pixel} proposes an image generation model PixelRNN \jr{$\leftarrow$ Cite the paper} which use prior pixels to predict current pixel. Each pixel $x_i$ is in turn jointly determined by three values, Red, Green and Blue, each of the colors is conditioned on the other channels
as well as on all the previously generated pixels. The architectures consist PixelCNN, Row LSTM, Diagonal BiLSTM, and Multiple residual blocks. 

In \textbf{text domain}, The GPT series is an auto-regressive model. At the stage of unsupervised pre-training, let $k$ be the size of the context window which means that using prior $k$ not all tokens to predict current token. And the conditional probability $P$ is modeled using a neural network with parameters. GPT-1 applies a multi-headed self-attention operation over the input context tokens followed by position-wise feed forward layers to produce an output distribution over target tokens.

\subsubsection{Flow-based Models.}

Flow-based Model is constructed by a series of reversible transformations. It use\jr{s} a series of reversible transformations $f_1, f_2, \dots, f_K$ to transfer a uni-modal distribution $\boldsymbol{z}$ to a complex real distribution $\boldsymbol{x}$ \jr{$x$ is used in previous text. Don't use one notation to represent different concepts in one paper.}. Using series of normalizing flow, repeatedly substitute the variable for the new one according to the change of variables theorem and eventually obtain a probability distribution of the final target variable. It clearly learned about data distribution, so the loss function is just negative log-likelihood. Represented through symbolization: $\boldsymbol{z}_{i-1} \sim p_{i-1}(\boldsymbol{z}_{i-1}), \boldsymbol{z}_{i}=f_i(\boldsymbol{z}_{i-1}), \boldsymbol{z}_{i-1}=f_i^{-1}(\boldsymbol{z}_{i})$, so we have \jr{Do we use these notations in the following paper? If we didn't use them in the following text, I think we don't need to present notations here.}
\begin{align*}
p_i(\boldsymbol{z}_{i})=p_{i-1}(f_i^{-1}(\boldsymbol{z}_{i}))\lvert \mathrm{det}\frac{\mathrm{d}f_i^{-1}}{\mathrm{d}\boldsymbol{z}_{i}} \rvert
\end{align*}
This kind of model is mainly used for image generation.

In \textbf{image domain}, \citet{dinh2016density} extend the space of such models using real-valued non-volume preserving (real NVP) transformations, a set of powerful, stably invertible, and learnable transformations, resulting in an unsupervised learning algorithm with exact log-likelihood computation, exact and efficient sampling, exact and efficient inference of latent variables, and an interpretable latent space. \citet{kingma2018glow} simplify the architecture by replacing reverse swapping operations on channel sorting with reversible 1x1 convolutions.


\subsubsection{Latent Variable Models.}

The idea behind latent variable models is to assume a lower-dimensional \jr{Diffusion model is not a lower-dimention} latent space and the following generative process:
$$
\boldsymbol{z}\sim p\left( \boldsymbol{z} \right) ,
\boldsymbol{x}\sim p\left( \boldsymbol{x}|\boldsymbol{z} \right) 
$$
It introduces latent variables to learn $p(\boldsymbol{x})$. This kind of models conclude VAE, GAN and Diffusion Models. Due to the fact that the process of generating an image is a process of transforming a random vector into an image, which is difficult to learn, VAE learns how to transform an image into a vector at the same time to make it easier. GAN train 2 networks for adversarial training, using discriminator to tell whether the generator generate a good sample. Diffusion model learn to reverse the process that adding noise to a real image until to a simple noise, and then can generate a real data from a noise.

1) VAE. \jr{Do not create list number by yourself. Always try to use latex code to itemize.}

The main idea of Variational Auto Encoder(VAE) is using neural networks to modeling 2 complex conditional probability density functions: inference network and generation network. Inference network is to estimate variational distribution $q(\boldsymbol{z}|\boldsymbol{x};\theta)$ where $\theta$ is the parameters of the network, $q$ is an additional introduced variational density function, $\boldsymbol{z}$ is the latent variables. Generation network is to estimate probability distribution $p(\boldsymbol{x}|\boldsymbol{z};\theta)$. By reparameterization, VAE can use gradient descent method to learn parameters, thereby improving the training efficiency.

2) GAN

Generative Adversarial Networks(GAN) is a kind of implicit density model because it don't explicitly model $p_r(\boldsymbol{x})$. In GAN, there are two networks for adversarial training. One is the discriminator network $D$, with the goal of accurately determining whether a sample is from real data or generated by the generative network as much as possible; The other is to generator network $G$, with the goal of generating as many samples as possible that the discriminative network cannot distinguish between sources. These two networks with opposite objectives continuously undergo alternating training until they converge to the point where the discriminative network cannot determine the source of a sample, meaning that the generative network can generate samples that match the true data distribution. The loss function is:
% GAN adversarial loss.
\begin{equation}\label{eq: gan}
    \begin{aligned}
    \min _G \max _D \mathbb{E}_{x \sim \mathcal{D}_{\text {data }}} \log D(x) +\mathbb{E}_{x \sim \mathcal{D}_G} \log (1-D(x))
    \end{aligned}
\end{equation}

3) Diffusion Models

The diffusion model consists of two parts: forward process and reverse process. The forward process is to add Gaussian noise to the real image for $T$ steps. And the reverse process is to remove the noise to reduction the real data. The forward process is a Markov Process which means that the current state is only determined by the state in front of it.
\begin{align*}
    q\left(\mathbf{x}_t \mid \boldsymbol{x}_{t-1}\right)=\mathcal{N}\left(\mathbf{x}_t ; \sqrt{1-\beta_t} \mathbf{x}_{t-1}, \beta_t \boldsymbol{I}\right)
    \label{eq:forward}
\end{align*}
It can be proved that, when the $\beta_t$ is small enough, the inverse operation of adding noise also satisfies a normal distribution, so, the training loss function is that let a predicted noise $\epsilon_\theta(\boldsymbol{x}_t,t)$ is close to the noise $\epsilon_t$ that added at the forward process.
\begin{align*}
\mathcal{L} = \left \| \epsilon_t-\epsilon_\theta(\boldsymbol{x}_t, t) \right \| ^2
\end{align*}
To lower the computational demands of training diffusion models towards high-resolution image synthesis, Stable Diffusion utilize an autoencoding model which learns a latent space $\boldsymbol{z}=\mathcal{E}(\boldsymbol{x})$ that is perceptually equivalent to the image space, but offers significantly reduced computational complexity. The loss function is as following
\begin{equation}
    \label{eq:sd_loss}
    \begin{aligned}
    \mathcal{L}_{\text{SD}}=\mathbb{E}_{\mathcal{E}(\boldsymbol{x}), c, \boldsymbol{\epsilon} \sim \mathcal{N}(0,1), t}\left[\left\|\boldsymbol{\epsilon}-\boldsymbol{\epsilon}_\theta\left(\boldsymbol{z}_t, c, t\right)\right\|^2\right]
    \end{aligned}
\end{equation}


\subsubsection{Energy-Based Models.}

Models defined by an energy function are referred to as energy-based models (EBMs). The main idea behind EBMs is to formulate the energy function $E(\boldsymbol{x})$ and calculate (or rather approximate) the partition function $Z=\sum_{\boldsymbol{x}}\mathrm{exp}\{-E(\boldsymbol{x})\}$. The largest group of EBMs consists of Boltzmann Machines that entangle $\boldsymbol{x}$’s through a bilinear form: $E(\boldsymbol{x})=\boldsymbol{x}^{\mathrm{T}}\boldsymbol{W}\boldsymbol{x}$. Introducing latent variables and taking $E(\boldsymbol{x}, \boldsymbol{z})=\boldsymbol{x}^{\mathrm{T}}\boldsymbol{W}\boldsymbol{z}$ results in Restricted Boltzmann Machines.

% I think it's better to introduce important model which in different domains on the previous part. There's no need to list all loss function for all model and their variant models. We just list the most import models which we may use below for protect functions is OK. So I first annotate the following formula. I'll add if there's need for the following part. 

% \textbf{Domains Perspective.}


% \textbf{i. Image.} The classic generative models in computer vision have led the development of DGMs, which contains important methods of Generative Adversarial Network (GAN), Variational auto-encoder (VAE), Flow-based models, and Diffusion-based model.



% VAE. Can also compress data.

% DDPM
% \begin{align}
%     p_\theta\left(\mathbf{x}_{t-1} \mid \mathbf{x}_t\right)=\mathcal{N}\left(\mathbf{x}_{t-1} ; \mu_\theta\left(\mathbf{x}_t, t\right), \Sigma_\theta\left(\mathbf{x}_t, t\right)\right)
%     \label{eq:reverse}
% \end{align}

% \begin{align*}
%     L=
%         \mathbb{E}_{\mathbf{x}_0, \boldsymbol{\epsilon}}\left[\frac{\beta_t^2}{2 \sigma_t^2 \alpha_t\left(1-\bar{\alpha}_t\right)}\left\|\boldsymbol{\epsilon}-\boldsymbol{\epsilon}_\theta\left(\sqrt{\bar{\alpha}_t} \mathbf{x}_0+\sqrt{1-\bar{\alpha}_t} \boldsymbol{\epsilon}, t\right)\right\|^2\right]
% \end{align*}

% \begin{align}
%     L^{\text {simple }}=\mathbb{E}_{t, \mathbf{x}_0, \boldsymbol{\epsilon}}\left[\left\|\boldsymbol{\epsilon}-\boldsymbol{\epsilon}_\theta\left(\sqrt{\bar{\alpha}_t} \mathbf{x}_0+\sqrt{1-\bar{\alpha}_t} \boldsymbol{\epsilon}, t\right)\right\|^2\right]
%     \label{eq:ddpm_simple_loss}
% \end{align}
% Stable Diffusion


% \textbf{ii. Text.} Transformer.

% \textbf{iii. Audio.}

\subsection{Copyrights in DGMs} \label{Copyrights in DGMs}
\jr{Maybe in Section 2 we don't need to introduce }

The copyright in Deep Generative models can mainly divided into 2 parts, data copyright and model copyright. The definition of copyrights and infringement upon copyrights are similar in different domains. So, in this part, we will draw a clear image of what is copyright and then talk about unique properties for specific domain in their own sections. Whether it's model copyright or data copyright, a copyright is a type of intellectual property that gives its owner the exclusive right to copy, distribute, adapt, display, and perform a creative work, usually for a limited time. And by the definition of \cite{lee2023language} , the violation of copyright means \textit{"the act of exploiting another person’s work or idea without referencing the individual as its author"}. With very powerful generation capabilities, Deep Generative Models have now attracted widespread attention, therefore, copyright protection is particularly important. We'll introduce copyright and possible infringement upon copyright for model and data.

\textbf{Model copyright.} The infringement on model copyright is consistent in different settings and data domains. It refers to the usage of the DGM without the permission from the model builder. Although the purpose of building a powerful model by the model builder is to help people to use it to generate some images, texts, audios, videos, graphs. And hope the generated data may help for learning some new things, getting some instructions, getting beautiful pictures to enjoy and so on. However, the model builder also pay a lot of efforts to collect, filter and process vast amount of data to train the model. And the training process also consumes a lot of energy and time, for instance, some large language models cost 2 million to 12 million dollars or even more. And building an excellent model framework is also a labor achievement of researchers. So, using models to generate data without permission is the infringement upon copyright. The unauthorized may use the published model, violating the licence for forbidden commercial or malicious targets. If the model parameter is not available, they can also call the API for the development of their own program without permission. In the other hand, the model may also be misused to generate unhealthy and harmful public content. For example, using large language models to generate fake news to induce the public, using DGMs to generate fake photos related to the president, and using DGMs to generate a voice to imitate someone's pronunciation for fraud. 


\textbf{Data copyright.} Because of the vast amount of data needed to train the DGMs, crawling from the internet is a common way to obtain data, thus posing a risk of copyright infringement because it is difficult to find the publisher one by one to obtain consent for such a large amount of data. Even worse, whether it's a large language model or a large image generation model or in other domains, the model may leak training data. This poses a risk of leaking personal privacy. In different domains, the levels of copyright infringement vary. From the strictest perspective, infringement is only considered when the output and training data of DGMs are identical or partially identical. For example, in a large language model, verbatim copying of training data is used as the output result. Alternatively, the generative images that are almost identical to the training set, although not all pixels are consistent, they describe almost the same content in human eyes. If the standards are slightly relaxed, the similarity in style and content is also an infringement of copyright. ~\citep{shan2023glaze, van2023anti} claim that if the generated images from a DGM trained on the copyrighted data share any similar semantic features with the copyrighted images like objects, textures and styles, it should be seen as the infringement. For text domain, same content or style may constitute infringement of copyright. The most widespread infringement standard is that unauthorized use of data constitutes copyright infringement. When the data owner claims copyright, model construction should eliminate the impact of the data on model training.

(However, it is crucial to note the relationship of memorization, membership inference, inversion and replication: A generative model that memorizes data might allow for model inversion or only membership inference, yet the same model might never spontaneously generate the training data by accident~\cite{somepalli2023diffusion})



\subsubsection{Data Owner (\sout{Hongzhi} This is not written by me. Who?)}

\han{Give the backgrounds. Are they the owner of datasets? Are they the owner of creative works? What is NTF? What is NFT? What is NDM????????????????}


\han{Give some motivations, backgrounds.}
\citet{ranjbar2023nft} proposed NTF-based data marketplace where data owners sell the data to the data buyers to protect the copyright. Digital watermarking  and blockchain are combined to protect the copyright \han{why does selling to them protect the copyright??}. Watermarking is used to embed owner and buyer information which can be extracted from the traded asset. And the proof of ownership for the data is stored as an NFT on a blockchain. Specifically, the data owner and buyer register in the marketplace, and get a unique id, then the data owner send their data onto the data storage server and the data will be embed messages including data owner and then be storaged as an NFT. After buying the data, the data will be transferred to the buyer before adding watermark with the information of buyer and owner. And using NDM the owners can observe and track all the transactions related to their listed data.

